Analyzing Encoded Concepts in Transformer Language Models

We propose a novel framework ConceptX, to analyze how latent concepts are encoded in representations learned within pre-trained language models. It uses clustering to discover the encoded concepts and explains them by aligning with a large set of human-defined concepts. Our analysis on seven transformer language models reveal interesting insights: i) the latent space within the learned representations overlap with different linguistic concepts to a varying degree, ii) the lower layers in the model are dominated by lexical concepts (e.g., affixation), whereas the core-linguistic concepts (e.g., morphological or syntactic relations) are better represented in the middle and higher layers, iii) some encoded concepts are multi-faceted and cannot be adequately explained using the existing human-defined concepts.

==> sections/compositional_concepts.tex <==
\begin{figure*}[t]
    \begin{subfigure}[b]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/ADJ+NN.png}
    \caption{}
    \label{fig:jj+nn}
    \end{subfigure}
    \begin{subfigure}[b]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/Albert-11-135.png}
    \caption{}
    \label{fig:vbforms}
    \end{subfigure}
    \centering
    \begin{subfigure}[b]{0.24\linewidth}
    \centering
     \includegraphics[width=\linewidth]{figures/BERT-c-1-316.png}
    \caption{}
    \label{fig:liwc}
    \end{subfigure}
    \centering
    \begin{subfigure}[b]{0.24\linewidth}
    \centering
    \includegraphics[width=\linewidth]{figures/NN+y.png}
    \caption{}
    \label{fig:nn+y}
    \end{subfigure}    
    % \centering
    % \begin{subfigure}[b]{0.24\linewidth}
    % \centering
    % \includegraphics[width=\linewidth]{figures/TV.png}
    % \caption{}
    % \label{fig:tv}
    % \end{subfigure}
    \caption{Clusters: (a) mBERT:Layer 9:830 = SEM:GPE + POS:JJ is a cluster representing countries and their adjectives, (b) ALBERT: Layer 11: 135 = POS:VBG + POS: VBN + POS:VBD (c) BERT-c: Layer 1: 316 = LIWC:negemo + LIWC:death, (d) mBERT:Layer 9:833 = POS:NN + Suffix:y is a cluster having nouns ending with suffix `y' %, (d) ALBERT: Layer 11: 562 POS:NNP + SEM:ORG
    }
    \label{fig:clusters}
\end{figure*}


\subsection{Compositional Concepts}
\label{sec:composition}

In the above section, we discussed the concepts that perfectly align with the 
human-defined concepts. 
%traditionally conceived linguistic concepts. 
Here we study 1$\rightarrow$M cases where an encoded concept can be mapped to multiple human-defined concepts. Such an analysis could be useful for two scenarios: i) to create explanations for the unaligned concepts, ii) to create fine-grained explanations for the already aligned concepts.

\paragraph{Unaligned Concepts:} %While some clusters strictly adhere to the traditionally conceived linguistic concepts as we observed in the above sections,
In Table \ref{tab:compCoverage}, we found that at least 27.6\% (in XLM-R) and up to 56.4\% (in XLNet) %-- See Table \ref{tab:coverage}) 
did not fully adhere to %of 
the encoded concepts. %were not aligned. 
\emph{What concepts do these unaligned clusters contain?} In an effort to answer this question, we analyzed if some of these clusters can be explained via compositions.
%the remaining clusters.  
%We observed that many of these clusters were compositional concepts that  simultaneously capture multiple dimensions of the words and often provide additional information that is not captured in traditionally defined human-concepts. 
%\textcolor{red}{Fahim can we get some statistics/plots on clusters composed of 2, 3, 4 etc clusters?}
Figure \ref{fig:jj+nn} shows an interesting unaligned concept in multilingual BERT which is composed from a semantic category (SEM:GPE -- geopolitical entity %(66.8\%) 
and a morphological category (POS:JJ -- adjective). %53.8\%). 
%While the two categories roughly describe the cluster, %but 
Using the composition of these two categories, we can get
an accurate description of this cluster i.e countries and their corresponding adjectives. %Moreover 
Another unaligned concept is shown in Figure \ref{fig:vbforms}, where a cluster is composed of different verb forms (past/present and gerunds). 
Lastly Figure \ref{fig:liwc} shows an encoded concept composed of two human-defined concepts LIWC:negative emotions %(84.16\%) 
and LIWC:death. %(15.38\%). 
Please also see Appendix (Figure \ref{tab:compCoverage}) where we quantitatively show how many unaligned concepts we can explain by
%how much coverage can be gained by 
allowing up to $N$ different concepts to form a cluster, with a criterion that 90\% of the words must cumulatively belong to these $N$ concepts.

\paragraph{Aligned Concepts} Compositionality is also helpful in discovering a finer explanation for already aligned concepts. Figure \ref{fig:nn+y} shows an example of an encoded concept that is aligned with %multiple concepts %but gives a more fine-grained view. %(marked as  POS:NN + Suffix:y) showing that 
%This %cluster 
%concept is composed of 
POS:NN, but the additional information Suffix:y enriches the explanation that %most of 
%the words in the cluster end with suffix ``y"
this encoded concept captures nouns ending with a suffix ``y'', %. The composition can be termed as Noun words ending with ``y'', 
a concept that is not found in human-defined ontology. 
Similarly, Figure~\ref{fig:jj+nn} has an additional geographic detail that the locations belong to the European region which is not captured by these tags.
%Similarly Figure \ref{fig:tv} shows a concept that has been auto-annotated as SEM:ORG and POS:NNP, but concept signifies additional information showing TV channels. 

%Lastly Cluster 892 is annotated as SEM:UOM i.e. as a unit of measurement. The cluster signifies more  fine-grained information of  measuring units for currency, specifically dollar, euros and pound symbols. 


==> sections/introduction_FA_HS.tex <==

Deep Neural Networks (DNNs) brought significant progress to NLP tasks. One major advancement of the deep learning approach is that it retains hidden features, a powerful means to extract new composition features from the data. Despite the benefits of DNNs, their black-box nature is a major cause of a concern, resulting in lack of explainability, reliability, and controllability.

A large number of research work aimed at interpreting DNNs and analyzed the knowledge learned in their representations with respect to linguistic properties 
%\jx{Shall we be consistent to the categories? or we need to explain human-defined concepts} 
% fixed
such as parts of speech tags (POS), semantic tags (SEM) and syntactic tags. A common approach to perform such an analysis is to gauge how well a linguistic property can be predicted using hidden representations of the model. Various works based on this approach showed that the representations posses the knowledge of linguistic properties~\cite{vylomova2016word, belinkov:2017:acl,voita-etal-2019-analyzing,tenney-etal-2019-bert,conneau2018you}.
%
%While the approach measures the knowledge of a human-defined concept in the representation, it does not reflect on how the knowledge is structured in the representation.
%They showed that the representations posses the knowledge of various human-defined concepts~\cite{vylomova2016word, belinkov:2017:acl,voita-etal-2019-analyzing,tenney-etal-2019-bert,conneau2018you}. 
In this work, we approach the interpretation of representations from a different angle. In contrast to relying on the prediction power of representations, we analyze how knowledge is structured within the representations in an unsupervised way. This leads of various questions such as, do representations encode knowledge inline with linguistic %human-defined 
properties such as POS, SEM?, which properties dominate the structure?, and are there novel properties exist beyond them? %human-defined properties? 
Answer to these questions reveals how DNNs structure language information to learn a task.

% A large number of research work aimed at interpreting DNNs and analyzed the knowledge learned in their representations with respect to human-defined concepts such as parts of speech tags (POS), semantic tags (SEM) and syntactic tags. They showed that the representations posses the knowledge of various human-defined concepts~\cite{vylomova2016word, belinkov:2017:acl,voita-etal-2019-analyzing,tenney-etal-2019-bert,conneau2018you}. 
% In this work, we approach the interpretation of representations from a different angle and we question how knowledge is structured within representations. This leads to various questions such as, do representations encode knowledge inline with human-defined concepts such as POS, SEM?, if yes, which categories dominate the structure?, and are there novel concepts exist beyond human-defined concepts?

%A common approach to perform such an analysis is to gauge how well a human-defined concept can be predicted using hidden representations of the model **cite**. While this approach measures the knowledge of a human-defined concept in the representation, it does not reflect on how the knowledge is structured in the representation. 
%Questions such as, does the representation encode knowledge in-line with human-defined categories? Do the structure of various human-defined categories present such as parts of speech and semantic tagging? Are there any new novel categories learned beyond human definition? 

%Post-hoc analysis of the representations learned within deep NLP models is one of the mainstream areas in interpretability. To this end, the researchers have analyzed what knowledge is learned within the representations through relevant extrinsic phenomenon varying from word morphology \cite{vylomova2016word, belinkov:2017:acl,dalvi:2017:ijcnlp} to high level concepts such as \fa{syntactic} structure \cite{shi-padhi-knight:2016:EMNLP2016,linzen2016assessing}  and semantics \cite{qian-qiu-huang:2016:P16-11, belinkov:2017:ijcnlp} or more generic properties such as sentence length \cite{adi2016fine,bau2018identifying}.

%A predominant framework for probing knowledge in neural models uses \emph{Diagnostic Classifiers} \cite{hupkes2018visualisation,conneau2018you}. The central idea is to extract feature representations from the network and train an auxiliary classifier to predict the property of interest. The quality of the trained classifier on the given task serves as a proxy to the quality of the extracted representations w.r.t to the understudied property \cite{belinkov-etal-2020-analysis}. Probing classifiers has been widely used to interpret the learned models, which has advantages and limitations \cite{10.1162/coli_a_00422}. In this study, we follow a different approach by focusing on latent representations and without training any probing classifier.
% The widely used probing framework is one line of research which has pros and cons. For e A pitfall to this approach is whether the probe is faithfully reflecting the property of the representation or just learned the task \cite{hewitt-liang-2019-designing}? Another concern is whether to use simple probes, such as linear classifiers or a more complex as advocated in some recent studies \cite{pimentel2020informationtheoretic}?
% }

% \textcolor{blue}{
% In this work, we present an alternative framework called as the \emph{\textcolor{red}{SOME FANCY NAME HERE}\fa{conceptX?} }. Rather than training an auxiliary classifier on the learned representations, we cluster the learned representations into hierarchies using agglomerative clustering~\citep{gowda1978agglomerative}. These clusters represent latent ontologies captured within the learned representations. We then align these ontologies with the classic linguistic ontologies as well as other human defined concepts to analyze the learned representations. \fa{In figure X, we provide an example of such concepts alignment.} Our approach does away from the proxy classifier and its specificities and directly focuses on the latent representations. We target questions such as:

To this end, we discover \textit{encoded concepts} 
%\jx{introduce?} 
learned in pre-trained models and compare them with \textit{human-defined concepts}. 
%\jx{categories}. we are staying with concepts
% 
%We introduce \textit{encoded concepts} to represent a latent relationship based on which a group of representations are clustered together in high-dimensional space. 
Our inspiration to use the term \textit{concept} came from \textit{``concept based explanation''}, which has been used in computer vision~\cite{kim2018interpretability,ghorbani2019towards,chen2020concept}.  
%\jx{added another recent citation}
%A few examples of concepts in images include ``curly'' hairstyles, ``striped'' patterns.
\newcite{stock2010concepts} defines concept as ``a class containing certain objects as elements, where the objects have certain properties''.
%
%We define \textit{encoded concepts} to represent ``a latent relationship based on which a group of representations are clustered together in high-dimensional space''.
\textit{We define an encoded concept as a cluster of context-aware latent representations of words, where the representations are encoder layer outputs.} 
\sout{Each representation is computed as the encoder output during the contextualized embedding of a word in the high dimensional vector space.} 
As illustrated in Figure~\ref{fig:encodedconcept}, a context of word is fed into Transformer~\cite{Vaswani:2017}, and each hidden layer in the encoder outputs a vector representation. % to predict the masked input word $w$. 
\hs{the point of masking is not correct in the case of generative models like XLNet}
For each layer, we group the vector representations of words using heap-based agglomerative clustering~\cite{gowda1978agglomerative}. 

%After generating our encoded concepts, we ask our first Research Question (\textit{\textbf{RQ}}).

\jx{it looks that there is no new research questions, now. are you sure we will delete them all?}

Moreover, we introduce the term \textit{human-defined concepts} as a suite of pre-defined categories including but not limited to linguistic categories (e.g., POS, SEM), shallow lexical properties (e.g. suffix, casing), lexical concepts (WordNet, \newcite{miller1995wordnet} and psycholinguistic concepts (LIWC, \newcite{pennebaker2001linguistic}).  
%\jx{I see. This should come before any other use of ''human-defined concepts''. First the definition, and then the usages.}
The selection of a diverse set of human-defined concepts for comparison enables us to cover various abstraction of language such as morphology, semantics, psycholinguistic, etc. The encoded concepts may represent one or more of these concepts.

% To this end, we propose the \texttt{AutoConcept} framework which allows us to compare encoded concepts within a model with a diverse suite of human-defined concepts.
We propose a framework, namely \texttt{AutoConcept}, which allows us to compare encoded concepts within a model with a diverse suite of human-defined concepts.
%Specifically, the framework extracts encoded concepts learned within a network using hierarchical clustering, and  aligns them with the human-defined concepts. 
The overlap between the encoded concepts and the human-defined concepts would serve as a proxy to the way knowledge is structured within a model.
%
%To interpret the pre-trained models with such \textit{human-defined linguistic concepts} we 
Specifically, the framework clusters latent representations using agglomerative hierarchical clustering~\citep{gowda1978agglomerative}. 
The resulting clusters represent encoded concepts captured within the learned representations. We then align them with the human-defined concepts. Figure~\ref{fig:encodedconcept} summarizes the overall precedure. 
%provides an example of the overall framework. concepts alignment procedure.
In Figure \ref{fig:concept_examles}, we present a few examples of human-defined concepts that are aligned with encoded concepts. 
\jx{Do we use any human effort for the concept alignment? If so, is it still auto? Shall we directly call it "concept alignment"?}
\jx{Shall put the figure of how to do the alignment of the autoconcept? These are results of the concepts that can be shown in the experimental results. Also, maybe we need to take care on the overlap of this paper with the ICLR submission.}
%The word-clouds in the figure are obtained from latent representations (see Section \ref{sec:methodology}), which are then automatically mapped with \textit{human-defined linguistic concepts}. 
%Our approach, \textit{conceptX}, 
% does away from the proxy classifier and its specificities and 
%directly focuses on the latent representations. While doing so address the following  questions:

%In an ideal scenario, human-defined concepts should cover all possible grouping of words to 
%Our motivation to use a diverse set of human-defined concepts is to consider various known angles of grouping words 
%resources is that one knowledge source of linguistic aspects can not capture the latent representation well. For example, WordNet does not have enough coverage of named entities, and LIWC can capture limited emotional aspects.

% Our inspiration to use the term \textbf{concept}\footnote{A concept represents a notion and can be viewed as a coherent fragment of knowledge. \cite{stock2010concepts} defines concept as ``a class containing certain objects as elements, where the objects have certain properties''.} 
% %to explain pre-trained models 
% came from ``concept based explanation'', which has been used in computer vision \cite{ghorbani2019towards,kim2018interpretability}. Examples of concepts in images include ``curly'' hairstyles, ``striped'' patterns. 

% To interpret the pre-trained NLP models, in this study, we use the term \textit{human-defined linguistic concepts}, as {\em (i)} lexical concepts defined in WordNet \cite{miller1995wordnet}, {\em (ii)} psycholinguistic concepts defined in Linguistic Enquery Word Count (LIWC) \cite{pennebaker2001linguistic}, {\em(iii)} shallow lexical properties such as character bigram, case markers, {\em(iv)} lexical tags (e.g., POS) {\em(v)} syntax (e.g., chunking), {\em(iv)} semantics tags (e.g., NER), and {\em(iv)} word position. The motivation of using such diverse resources is that one knowledge source of linguistic aspects can not capture the latent representation well. For example, WordNet does not have enough coverage of named entities, and LIWC can capture limited emotional aspects. 


% A concept represents a notion and can be viewed as a coherent fragment of knowledge. \cite{stock2010concepts} defines concept as ``a class containing certain objects as elements, where the objects have certain properties''. ~\cite{deveaud2014accurate}  considers latent concepts as words that convey the most information or that are the most relevant to the initial query. A concept in language can be anything ranging from a shallow lexical property such as character bigram, to a complex syntactic phenomenon such as a adjectival phrase or a semantic property such as an event. Here, we loosely define concept as \textbf{\textit{a group of words that are meaningful}} where meaningful can be a lexical, semantic, syntactic, morphological and/or any other relationship. For example, names of ice-hockey teams form a semantic cluster, words that occur in a certain position of a sentence represent a syntactic concept, words that are first person singular verbs form a morphological cluster, words that begin with "anti" form a lexical cluster. In our implementation, we consider clusters of word contextual representations in BERT as hidden concept candidates and the human-annotated candidates with linguistic meanings as our discovered hidden concepts.

%, and generates new fine-grained types to enrich low-resource language analysis.

\begin{figure*}[!t] 
\begin{center}
        \includegraphics[width=1\textwidth]{figures/conceptpool.png}
      \caption{Encoded Concepts}
        \label{fig:encodedconcept}
        \end{center}
\end{figure*}

%\begin{figure}[!t] 
%        \includegraphics[width=0.5\textwidth]{figures/encodedconcept.jpeg}
%      \caption{Encoded Concepts}
%        \label{fig:encodedconcept}
%\end{figure}

\begin{figure}[tbh]
\centering
        \begin{subfigure}[b]{0.30\textwidth}
        \includegraphics[width=\textwidth]{figures/example1.png}
        \caption{SEM (NE - place names); LEX (title case)}
        \label{fig:example1}
    \end{subfigure}
    % \hfill
    %
    \begin{subfigure}[b]{0.30\textwidth}
        \includegraphics[width=\textwidth]{figures/example2.png}
        \caption{POS (NNP); SEM (NE - person names)}
        \label{fig:example2}
    \end{subfigure}
    % \hfill
    %
    \begin{subfigure}[b]{0.30\textwidth}
        \includegraphics[width=\textwidth]{figures/example3.png}
        \caption{WordNet (noun.person); POS (NNP); LEX (hyphenated names); SEM (NE - last names of person); LEX (title case)}
        \label{fig:example3}
    \end{subfigure}    
    \caption{Examples of human-defined linguistic concepts aligned with latent concepts. SEM: Semantic, LEX: lexical, NE: named entities.}
    \label{fig:concept_examles}
\end{figure}

% \begin{itemize}
% \itemsep=-1ex
% % \textcolor{blue}{
%     \item How much do the latent concepts learned in the pre-trained models align with the traditional human-defined linguistic concepts.
%     \item How do these concepts spread across different layers in the network?
%     \item How do different pre-trained models vary in learning different linguistic concepts?
%     \item How do architectures differ in their learned ontologies? 
%     \item Do multilingual models learn information differently?
%     % }
% \end{itemize}

We analyze eight pre-trained models with varying architectures, monolingual and multilingual training data, and with different case settings (e.g., large vs. small) using \texttt{AutoConcept}. Some notable findings of the analysis are as follows:

\begin{itemize}
    \item The lower layers encoded concepts are dominated by shallow lexical concepts such as suffixes.
    \item The middle-higher layers encode linguistic structure i.e., morphology, semantics and syntax.
    \hs{we need to probe this results further}
    \item The lower layers are rich in encoding WordNet and psycholinguistic-based concepts.
    \item The models learn novel concepts that do not adhere to human-defined concepts.
\end{itemize}

\jx{I don't see too often two item lists next to each other at the end of introduction. So maybe we can rearrange them in some other way?}

In summary, our contributions mainly lies in the following aspects:

\begin{itemize}
\item We introduce the \texttt{AutoConcept} framework to interpret encoded concepts learned in representations with respect to human-defined concepts.
\item We provide an empirical evidence of how knowledge is structured within a representation with respect to a large suite of human-defined concepts
\item We provide the \texttt{AutoConcept Tool} that facilitates the analysis of pre-trained models 
\end{itemize}

\jx{The introduction of ``encoded concept'' is the basis of all analysis that can be added to the contribution}

% \textcolor{red}{
% Our experimental evidence shows that the latent concepts largely agree with the human-defined linguistic concepts such as POS, Combinatory Categorial Grammar (CCG) \cite{hockenmaier2007ccgbank}, and wordnet. For example, in a lower layer, uppercased words are located close to each other in the vector space, and in a higher layer, words are gathered more based on their syntactic relationship, such as nouns, verbs, etc. This gives strong evidence of our assumption that latent representations of the pre-trained models learn the linguistic concepts.
% % , and with the increase of the layer, the features learned are more complex. % This result partially explains the link between features in rule-based, statistical-based NLP methods and those in NN. 
% % Furthermore, we generate many new concepts beyond the pre-defined linguistic categories,  which partially explains why NN-NLP outperforms the traditional rule-based, statistical-based NLP.
% }

% % \textcolor{blue}{
% To this end, we align latent concepts in various transformer models such as BERT \cite{devlin2018bert}, RoBERTa \cite{liu2019roberta}, XLNet \cite{yang2019xlnet}, AlBERT \cite{lan2019albert} and the multilingual models such as mBERT and XLM-RoBERTa \cite{xlm-roberta} with \textit{human-defined linguistic concepts} using \textcolor{red}{conceptX}. Our results show interesting findings such as: i) lower layers learn shallow lexical concepts such as affixes and ngrams, ii) subsequent layers in the model capture abstract ontologies such as morphology, syntax and semantics that are consistently found in the higher layers of the network, iii) ..., iv) ...
% % }


%%%%%%%%%%%%%%%%%

% This paper introduces encoded concepts to explain the meaning of hidden nodes learned in NLP Deep Learning models, compares them with human-defined linguistic categories, and generates new fine-grained types to enrich low-resource language analysis. 

% Deep Neural Networks (NN) brought significant progress to NLP tasks.  One major advance of the deep learning approach is that it retains hidden features, a powerful means to extract new composition features from the data. However, the meaning of NN's hidden layers is unknown due to its black-box nature, resulting in predictions lacking explainability, reliability, and controllability. There is a critical need to understand whether (and if yes, what kind of) linguistic rules/phenomena are learned as hidden features and how they contribute to the final prediction. 

% In tandem with the expansion of deep learning in various domains and applications, extensive work has been done in NN interpretation~\cite{}. Some of the core questions considered in these posthoc analyses of neural networks include: ``What concept (ordinary ideas or general notions) does a unit in a hidden layer of a trained neural network represent and does this unit in the network represent a concept that a human might understand?''~\cite{chen2020concept}. 
% \hs{I would stay away from prediction and decision part since our analysis is also independent of the prediction}
% A common belief is that hidden nodes presumably learn surface features in lower-level layers and composite and complex features in higher-level layers~\cite{gu2018recent}. Yet, in NLP, such an assumption is hard to verify because it is impossible to trace how  millions and billions of neuron parameters combine to make decisions. 


% \begin{figure}[!t] 
%         \includegraphics[width=0.5\textwidth]{figures/encodedconcept.jpeg}
%       \caption{Encoded Concepts}
%         \label{fig:encodedconcept}
% \end{figure}


% We overcome this limitation by introducing "encoded concept".  \textit{An encoded concept is a cluster of context-aware representations of words.} Such a vector representation is computed as the encoder output during contextualized word embedding, indicating the feature attributes of a word. \hs{is a cluster of contextualized word embedding}The vector space of each encoding layer contains a set of encoded concepts. As illustrated in Figure~\ref{fig:encodedconcept}, our approach utilizes the BERT~\cite{} based on Transformer~\cite{}. A context of 251-word window size is fed into BERT, and each hidden layer in the encoder outputs an encoding vector representation to predict the masked input word $w$. We group the encoded vector representations of different words given a layer using heap-based agglomerative clustering~\cite{}. After generating our encoded concepts, we ask our first Research Question (\textit{\textbf{RQ}}).

% \textit{\textbf{RQ1}: How do encoded concepts learned in BERT compare with human-defined linguistic categories?}

% We consider a wide range of pre-defined categories, from linguistic concepts, psycho-linguistic concepts to shallow concepts. We use POS, CCG, and wordnet tags/schemes. 
% Our experimental evidence shows that our encoded concepts largely agree with the human-defined categories, including POS, CGG, wordnets. For example, in a lower layer, uppercased words are located close to each other in the vector space, and in a higher layer, words are gathered more based on their syntactic relationship, such as nouns, verbs, etc.  This gives strong evidence of our assumption that NN hidden nodes learn the linguistic properties, and with the increase of the layer, the features learned are more complex. This result partially explains the link between features in rule-based, statistical-based NLP methods and those in NN. Furthermore, we generate many new concepts beyond the pre-defined linguistic categories,  which partially explains why NN-NLP outperforms the traditional rule-based, statistical-based NLP. Thus, we further ask: 


% \textit{\textbf{RQ2}: Are there any new useful concepts we learned from NN beyond human definition?}

% We have found new concepts beyond the traditional linguistic categories from POS, CCG, etc.
% We found new composite concepts and a mix of various pre-defined concepts, highlighting a possibility to enrich pre-defined concepts. These concepts are usually fine-grained concepts describing new linguistic word groups such as soccer player names. Our approach has the advantage of finding novel  concepts dynamically given the data vary  over time and domains, thus being more suitable to serve NLP applications. Most importantly, we do not need any human linguistic labeling. Given above advantages, we finally ask:

% \textit{\textbf{RQ3}:  How can concept findings be helpful for low-resource annotations?}

% Many low-resource languages do not have enough labels for linguistic analysis (check the terms), such as POS, CCG, etc. This greatly hindered the NLU tasks due to a lack of linguistic resources. We show that our encoded concepts can automatically extract linguistic categories on monolingual text without any human labeling for specific linguistic analysis tasks that can be expensive and rare to find. Furthermore, we apply transfer learning and further boost those encoded concept finding accuracy by incorporating bilingual corpus with English.

% In summary, our contribution mainly lies in the following aspects:
% \begin{enumerate}
% \item Introduce a new method, called ``encoded concept", explaining hidden nodes' meaning in NN-based NLP models.
% \item Measure the consistency of the human-defined linguistic categories and the encoded concepts learned from NN.
% \item Empirical evidence of the feature types (shallow versus complex) learned in different levels of NN hidden layers.
% \item Find new concepts beyond the existing human-defined linguistic categories.
% \item Enrich existing linguistic resources with our unsupervised learning of encoded concepts.
% \end{enumerate}


==> sections/introduction_jia.tex <==
\section{Introduction (by Jia)}
This paper introduces encoded concepts to explain the meaning of hidden nodes learned in NLP Deep Learning models, compares them with human-defined linguistic categories, and generates new fine-grained types to enrich low-resource language analysis. 

Deep Neural Networks (NN) brought significant progress to NLP tasks.  One major advance of the deep learning approach is that it retains hidden features, a powerful means to extract new composition features from the data. However, the meaning of NN's hidden layers is unknown due to its black-box nature, resulting in predictions lacking explainability, reliability, and controllability. There is a critical need to understand whether (and if yes, what kind of) linguistic rules/phenomena are learned as hidden features and how they contribute to the final prediction. 

In tandem with the expansion of deep learning in various domains and applications, extensive work has been done in NN interpretation~\cite{}. Some of the core questions considered in these posthoc analyses of neural networks include: ``What concept (ordinary ideas or general notions) does a unit in a hidden layer of a trained neural network represent and does this unit in the network represent a concept that a human might understand?''~\cite{chen2020concept}. 
\hs{I would stay away from prediction and decision part since our analysis is also independent of the prediction}
A common belief is that hidden nodes presumably learn surface features in lower-level layers and composite and complex features in higher-level layers~\cite{gu2018recent}. Yet, in NLP, such an assumption is hard to verify because it is impossible to trace how  millions and billions of neuron parameters combine to make decisions. 


\begin{figure}[!t] 
        \includegraphics[width=0.5\textwidth]{figures/encodedconcept.jpeg}
       \caption{Encoded Concepts}
        \label{fig:encodedconcept}
\end{figure}


We overcome this limitation by introducing "encoded concept".  \textit{An encoded concept is a cluster of context-aware representations of words.} Such a vector representation is computed as the encoder output during contextualized word embedding, indicating the feature attributes of a word. \hs{is a cluster of contextualized word embedding}The vector space of each encoding layer contains a set of encoded concepts. As illustrated in Figure~\ref{fig:encodedconcept}, our approach utilizes the BERT~\cite{} based on Transformer~\cite{}. A context of 251-word window size is fed into BERT, and each hidden layer in the encoder outputs an encoding vector representation to predict the masked input word $w$. We group the encoded vector representations of different words given a layer using heap-based agglomerative clustering~\cite{}. After generating our encoded concepts, we ask our first Research Question (\textit{\textbf{RQ}}).

\textit{\textbf{RQ1}: How do encoded concepts learned in BERT compare with human-defined linguistic categories?}

We consider a wide range of pre-defined categories, from linguistic concepts, psycho-linguistic concepts to shallow concepts. We use POS, CCG, and wordnet tags/schemes. Our experimental evidence shows that our encoded concepts largely agree with the human-defined categories, including POS, CGG, wordnets. For example, in a lower layer, uppercased words are located close to each other in the vector space, and in a higher layer, words are gathered more based on their syntactic relationship, such as nouns, verbs, etc.  This gives strong evidence of our assumption that NN hidden nodes learn the linguistic properties, and with the increase of the layer, the features learned are more complex. This result partially explains the link between features in rule-based, statistical-based NLP methods and those in NN. Furthermore, we generate many new concepts beyond the pre-defined linguistic categories,  which partially explains why NN-NLP outperforms the traditional rule-based, statistical-based NLP. Thus, we further ask: 


\textit{\textbf{RQ2}: Are there any new useful concepts we learned from NN beyond human definition?}

We have found new concepts beyond the traditional linguistic categories from POS, CCG, etc.
We found new composite concepts and a mix of various pre-defined concepts, highlighting a possibility to enrich pre-defined concepts. These concepts are usually fine-grained concepts describing new linguistic word groups such as soccer player names. Our approach has the advantage of finding novel  concepts dynamically given the data vary  over time and domains, thus being more suitable to serve NLP applications. Most importantly, we do not need any human linguistic labeling. Given above advantages, we finally ask:

\textit{\textbf{RQ3}:  How can concept findings be helpful for low-resource annotations?}

Many low-resource languages do not have enough labels for linguistic analysis (check the terms), such as POS, CCG, etc. This greatly hindered the NLU tasks due to a lack of linguistic resources. We show that our encoded concepts can automatically extract linguistic categories on monolingual text without any human labeling for specific linguistic analysis tasks that can be expensive and rare to find. Furthermore, we apply transfer learning and further boost those encoded concept finding accuracy by incorporating bilingual corpus with English.

In summary, our contribution mainly lies in the following aspects:
\begin{enumerate}
\item Introduce a new method, called ``encoded concept", explaining hidden nodes' meaning in NN-based NLP models.
\item Measure the consistency of the human-defined linguistic categories and the encoded concepts learned from NN.
\item Empirical evidence of the feature types (shallow versus complex) learned in different levels of NN hidden layers.
\item Find new concepts beyond the existing human-defined linguistic categories.
\item Enrich existing linguistic resources with our unsupervised learning of encoded concepts.
\end{enumerate}


==> sections/introduction_nadir.tex <==

Contextualized word representations learned in transformer-based language models capture rich concepts making them ubiquitous for
transfer learning towards downstream NLP. Despite their revolution, the black-box nature of the deep NLP models is a major cause of concern. Understanding the inner dynamics of these models is important to ensure fairness, robustness, reliability and control. 

A plethora of research has been carried to probe DNNs for the linguistic knowledge (e.g. morphology, syntactic and semantic roles) captured within the learned representations. A commonly used framework to gauge how well linguistic information can be extracted
from these models is the \emph{Probing Framework} \cite{hupkes2018visualisation}, where we train an auxiliary classifier to predict the property of interest. To this end, the researchers have analyzed what knowledge is learned within the representations through relevant extrinsic phenomenon varying from word morphology \cite{vylomova2016word,belinkov:2017:acl,dalvi:2017:ijcnlp} to high level concepts such as \fa{syntactic} structure \cite{shi-padhi-knight:2016:EMNLP2016,linzen2016assessing}  and semantics \cite{qian-qiu-huang:2016:P16-11,belinkov:2017:ijcnlp} or more generic properties such as sentence length \cite{adi2016fine,bau2018identifying}.

In this work, we present a novel framework that we call as \texttt{ConceptAlign}. In contrast to relying on the prediction capacity of representations, we analyze how knowledge is structured within the representation in an unsupervised fashion. Specifically, the framework clusters latent representations using agglomerative hierarchical clustering~\citep{gowda1978agglomerative}. The resulting clusters represent \emph{encoded concepts} captured within the learned representations. We then align these latent concepts with the \emph{human-defined concepts} using an alignment function that measures the amount of overlap.

Our inspiration to use the term \textit{concept} came from \textit{``concept based explanation''} in computer vision~\cite{kim2018interpretability,ghorbani2019towards,chen2020concept}. \newcite{stock2010concepts} defines concept as ``a class containing certain objects as elements, where the objects have certain properties''. We define an \emph{encoded concept} as a cluster of context-aware latent representations of words, where the representations are the output of a neural network module (e.g. encoder layer or self-attention network).

We carry out our study on seven pre-trained models with varying optimization function, architecture, training data etc. We use a range of pre-defined linguistic categories (that we call as human-defined concept in this paper) such as shallow lexical properties (e.g. suffix, casing) or more abstract concepts e.g. 
morphological, syntactic, semantic or psycholinguistic concepts \cite{pennebaker2001linguistic}. Such diverse set of human-defined concepts for alignment, enable us to cover various abstractions of language. Some notable findings from our analysis are as follows:

\begin{itemize}
    \item Shallow linguistic concepts such as lexical ngrams or suffixes are predominantly captured in the lower layers of the network.
    \item We also found WordNet\cite{miller1995wordnet} and psycholinguistic-based concepts to be learned in the lower layers.
    \item Middle and higher layers encode concepts that capture abstract linguistic properties such as morphology, semantics and syntax. 
    \item We found that roughly 50\% of the encoded concepts adhere to our suite of human-defined concepts.
    \item The models learn novel concepts that do not adhere to human defined concepts.
\end{itemize}

Our contribution in this paper are as follow: i) We introduce an alternative framework called as \texttt{ConceptAlign} that interpret encoded concepts in the learned represention by aligning them to the human-defined concept. ii) We provide a qualative and quantative evidence of how knowledge is structured within deep NLP models with respect to a large suite of human-defined concepts. 

% \textcolor{blue}{Post-hoc analysis of the representations learned within deep NLP models is one of the mainstream areas in interpretability. To this end, the researchers have analyzed what knowledge is learned within the representations through relevant extrinsic phenomenon varying from word morphology \cite{vylomova2016word, belinkov:2017:acl,dalvi:2017:ijcnlp} to high level concepts such as \fa{syntactic} structure \cite{shi-padhi-knight:2016:EMNLP2016,linzen2016assessing}  and semantics \cite{qian-qiu-huang:2016:P16-11, belinkov:2017:ijcnlp} or more generic properties such as sentence length \cite{adi2016fine,bau2018identifying}.}

% \textcolor{blue}{A predominant framework for probing knowledge in neural models uses \emph{Diagnostic Classifiers} \cite{hupkes2018visualisation,conneau2018you}. The central idea is to extract feature representations from the network and train an auxiliary classifier to predict the property of interest. The quality of the trained classifier on the given task serves as a proxy to the quality of the extracted representations w.r.t to the understudied property \cite{belinkov-etal-2020-analysis}. A pitfall to this approach is whether the probe is faithfully reflecting the property of the representation or just learned the task \cite{hewitt-liang-2019-designing}? Another concern is whether to use simple probes, such as linear classifiers or a more complex as advocated in some recent studies \cite{pimentel2020informationtheoretic}?}

% \textcolor{blue}{In this work, we present an alternative framework called as the \emph{\textcolor{red}{SOME FANCY NAME HERE}\fa{conceptX?} }. Rather than training an auxiliary classifier on the learned representations, we cluster the learned representations into hierarchies using agglomerative clustering~\citep{gowda1978agglomerative}. These clusters represent latent ontologies captured within the learned representations. We then align these ontologies with the classic linguistic ontologies as well as other human defined concepts to analyze the learned representations. \fa{In figure X, we provide an example of such concepts alignment.} Our approach does away from the proxy classifier and its specificities and directly focuses on the latent representations. We target questions such as:}

% % \textcolor{blue}{

% \begin{itemize}
%     \item How much do the latent concepts learned in the transformer models align with the traditional linguistic concepts.
%     \item How do these concepts spread across different layers in the network?
%     \item How do different pre-trained models vary in learning different linguistic concepts?
%     \item How do architectures differ in their learned ontologies? 
%     \item Do multilingual models learn information differently?
% \end{itemize}

% % }

% \textcolor{blue}{
% To this end, we align ontologies in various transformer models such as BERT \cite{devlin2018bert}, RoBERTa \cite{liu2019roberta}, XLNet \cite{yang2019xlnet}, AlBERT \cite{lan2019albert} and the multilingual models such as mBERT and XLM-RoBERTa \cite{xlm-roberta} using \textcolor{red}{Our Method Name}. Our results show interesting findings such as: i) lower layers learn shallow lexical concepts such as affixes and ngrams, ii) subsequent layers in the model capture abstract ontologies such as morphology, syntax and semantics that are consistently found in the higher layers of the network, iii) ..., iv) ...
% }

% % \textbf{Questions}
% % 1. How does latent concepts learned in Transformer models compare with pre-defined concepts
% % 2. What are the novel concepts found?
% % 3. How concept findings can be helpful for low-resource annotations

% % \textbf{What we considered}
% % For 1, we compare linguistic concepts, psycho-linguistic concepts, and shallow concepts. 
% % For 2, we found composite concepts and a mix of various pre-defined concepts, highlighting a possibility to enrich pre-defined concepts
% % For 3, we are not sure yet.

% % \textbf{Results}
% % - Full network comparison with pre-defined concepts
% % - Layer-wise plots of pre-defined concepts 
% % - Comparison of Coarse pre-defined concepts
% % - Compare Cased vs. uncased models
% % - Compare multilingual vs. monolingual models
% % - Compare architectures
% % - Examples of Composite concepts

